A Tuning-Free Primal-Dual Splitting Algorithm for Large-Scale Semidefinite Programming

This paper proposes and analyzes a tuning-free variant of Primal-Dual Hybrid Gradient (PDHG), and investigates its effectiveness for solving large-scale semidefinite programming (SDP). The core idea is based on the combination of two seemingly unrelated results: (1) the equivalence of PDHG and Douglas-Rachford splitting (DRS); (2) the asymptotic convergence of non-stationary DRS. This combination provides a unified approach to analyze the convergence of generic adaptive PDHG, including the proposed tuning-free algorithm and various existing ones. Numerical experiments are conducted to show the performance of our algorithm, highlighting its superior convergence speed and robustness in the context of SDP.

==> Conclusion.tex <==
\section{Future Works}
\label{sec:conc}


    

    
    


==> Preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}
%This paper adopts the notation of resolvent $J_{A} \coloneqq (\mathbb{I}+A)^{-1}$ from \cite{douglas1956numerical}. Note that if $A = \partial f$, then $J_{\partial f} = \text{Prox}_{f}$. Let $\mathbb{S}_{+}^{n\times n}$ be the set of all $n \times n$ symmetric positive semi-definite matrix. Given $A,B\in \mathbb{R}^{n \times n}$, define operation $\langle A, B\rangle \coloneqq \sum_{i=1}^{n}\sum_{j=1}^{n} A_{ij}B_{ij}$. Define a linear mapping $\mathcal{A} \colon \mathbb{S}^{n\times n} \to \mathbb{R}^m$ as $\mathcal{A}(X) = 
%\begin{pmatrix}
%\langle A_1, X \rangle \\
%\langle A_2, X \rangle \\
%\vdots \\
%\langle A_m, X \rangle \\
%\end{pmatrix}$, where $A_1, A_2,\dots, A_m \in \mathbb{S}^{n\times n}$. Its adjoint mapping $\mathcal{A}^T \colon \mathbb{R}^m \to \mathbb{S}^{n\times n}$ is then defined as $\mathcal{A}^T(y)=\sum_{i=1}^{m}y_i A_i$. 

%SDP is of the form:
%\begin{equation}
%\label{prob:primal_sdp}
%\begin{aligned}
%\min_{X} \quad & \langle C, X \rangle\\
%\textrm{s.t.} \quad & \mathcal{A}(X) = b \\
%  & X \in  \mathbb{S}_{+}^{n\times n}   
%\end{aligned}
%\end{equation}
%whose goal is to minimize a linear objective function subject to $m$ linear equality constraints. 
%Its dual problem is of the form:
%\begin{equation}
%\label{prob:dual_sdp}
%\begin{aligned}
%\max_{y,S} \quad & b^Ty\\
%\textrm{s.t.} \quad & \mathcal{A}^T(y) \preceq C\\   
%\end{aligned}
%\end{equation}

%PDHG \cite{chambolle2011first} solves 
%$$
%\min_{x} f(x) + g(Ax)
%$$
%or the following saddle-point problem:
%\begin{align*}
%\min_{x} \max_{y} f(x) + y^TAx - g(y)
%\end{align*}
%It updates iterates as follows:
%\begin{align*}
%    &x^{k+1} = \text{Prox}_{\alpha f}(x^k - \alpha A^Ty^k) \notag\\
%    &y^{k+1} = \text{Prox}_{\beta g^*}(y^k + \beta A(2x^{k+1}-x^k))
%\end{align*}
%The optimality conditions are
%\begin{align*}
%    & 0 \in \partial f(x^*) + A^Ty^* \\
%    & 0 \in \partial g(y^*) - Ax^*.
%\end{align*}
%This motivates us to define the primal and dual residuals:
%\begin{align*}
%    & p(x,y) = \partial f(x) + A^Ty \\
%    & d(x,y) = \partial g(y) - Ax.
%\end{align*}
%We can measure the convergence by tracking the size of the these residuals. Note that the residuals are in general, multi-valued. We can obtain explicit formulas for these residuals by considering the update of PDHG with the following forms:
%\begin{align*}
%    &\text{Find}\ x^{k+1}\quad \text{s.t.}\quad 0 \in \partial f(x^{k+1}) + A^Ty^{k} + \frac{1}{\alpha_k}(x^{k+1}-x^{k}) \\
%    &\text{Find}\ y^{k+1}\quad \text{s.t.}\quad 0 \in \partial g(y^{k+1}) - A(2x^{k+1}-x^k) + \frac{1}{\beta_k}(y^{k+1}-y^{k}).
%\end{align*}
%This form of update yields:
%\begin{align*}
%    & p^{k+1} = \frac{1}{\alpha_k}(x^k-x^{k+1})-A^T(y^k-y^{k+1}) \in \partial f(x^{k+1}) + A^Ty^{k+1} = p(x^{k+1},y^{k+1})\\
%    & d^{k+1} = \frac{1}{\beta_k}(y^k-y^{k+1})-A(x^k-x^{k+1}) \in \partial g(y^{k+1}) + Ax^{k+1} = d(x^{k+1},y^{k+1})
%\end{align*}
%We say PDHG converges if 
%\begin{align*}
%\lim_{k\to\infty} \norm{p^k}^2 + \norm{d^k}^2 = 0.
%\end{align*}





==> Related_Work.tex <==
\section{Related Work}
\label{sec:related-work}
%\subsection{Scalable algorithms for SDP}
%The impracticality of interior-point methods for large-scale SDP has spurred the development of scalable SDP algorithms (refer to \cite{majumdar2019survey, lemon2016low} for exhaustive surveys). One approach is based on based on augmented Lagrangian paradigms \cite{yang2015sdpnal+, zhao2010newton}, particularly the ADMM \cite{wen2010alternating,zheng2020chordal, garstka2021cosmo, o2016conic, sun2020sdpnal+,zhao2010newton}. However, the least cheap implementation of this approach requires a full eigendecomposition in each iteration to project the iterate onto the positive semidefinite cone. Efforts have been made to develop projection-free algorithms that eliminate the need for computing full eigenvalue decomposition. Two well-known projection-free approaches are Frank-Wolfe method \cite{hazan2008sparse, yurtsever2019conditional} and Burer-Monteiro method \cite{burer2003nonlinear, burer2005local}. The former only necessitates a single coarse eigenvector computation per iteration, but convergence speed is relatively slow and more assumptions are needed to theoretically guarantee convergence. The latter employs factorization techniques to eliminate the conic constraint in SDP, at the expense of losing convexity. Further enhancements to the Burer-Monteiro method have been proposed, using block-coordinate updates \cite{wang2017mixing, erdogdu2022convergence} and Riemannian optimization techniques \cite{boumal2016non, journee2010low}. Moreover, to address storage challenges in large-scale SDP, \cite{yurtsever2017sketchy, ding2021optimal, yurtsever2021scalable} have drawn upon sketching tools from randomized numerical linear algebra to control SDP's storage costs.

%The most related work to ours is \cite{souto2022exploiting}. If we fix the primal and dual step sizes, our algorithm reduces to theirs. However, their work derives the algorithm using the generalized proximal point method, whereas we use the Douglas-Rachford method. Furthermore, our numerical experiments show superior performance over \cite{souto2022exploiting}'s.

%\subsection{PDHG and its adaptive variants}
%This paper contributes to this research domain by demonstrating that the PDHG method can solve SDP effectively at scale. PDHG is an operator splitting method originally designed for image processing applications \cite{chambolle2011first, condat2013primal}. Recently, it has been investigated to solve large-scale LP \cite{applegate2021practical} and CQP \cite{lu2023practical}, in which the most expensive operation is (sparse) matrix multiplication. PDHG-based LP has also been shown to better exploiting parallelization and memory usage \cite{lu2023cupdlp}. While extending PDHG to solve SDP is simple, the focus of this paper is to investigate its adaptive variants with provably convergent guarantees.

%PDHG with adaptive stepsizes has been a topic of interest in past studies. The balancing technique proposed by \cite{goldstein2013adaptive, goldstein2015adaptive} aims to adjust the ratio between the primal and dual step sizes, keeping the primal and dual residuals approximately equal. The idea of balancing primal and dual residuals has been further extended by \cite{yokota2017efficient,zdun2021fast} to take into account the local variation of gradient directions. A line search technique for automating the step size tuning has been suggested by \cite{malitsky2018first}. Inspired by \cite{o2020equivalence} that shows PDHG as an instance of DRM, we automate the step size in our approach by using tools from non-stationary DRM \cite{lorenz2019non, lorenz2023degenerate}.


